Stochastic excitation of internal gravity waves in rotating late F-type stars: A 3D simulation approach

There are no strong constraints placed thus far on the amplitude of internal gravity waves (IGWs) that are stochastically excited in the radiative interiors of solar-type stars. Late F-type stars have relatively thin convective envelopes with fast convective flows and tend to be fast rotators compared to solar-type stars of later spectral types. These two elements are expected to directly impact the IGW excitation rates and properties. We want to estimate the amplitude of stochastically excited gravity modes (g-modes) in F-type stars for different rotational regimes. We used the ASH code to perform 3D simulations of deep-shell models of 1.3 $M_\odot$ F-type solar-type stars, including the radiative interior and the shallow convective envelope. The IGWs are excited by interface interactions between convective plumes and the top of the radiative interior. We were able to characterise the IGWs and g-mode properties in the radiative interior, and we compared these properties using the computation from the 1D oscillation code GYRE. The amplitude of low-frequency modes is significantly higher in fast-rotating models and the evolution of the period spacing of consecutive modes exhibits evidence of a behaviour that is modified by the influence of the Coriolis force. For our fastest rotating model, we were able to detect the intermediate degree g-mode signature near the top of the simulation domain. Nevertheless, the predicted luminosity perturbations from individual modes still remain at small amplitudes. We obtained mode amplitudes that are several orders of magnitude higher than those of prior 3D simulations of solar models. Our simulations suggest that g-mode signatures could be detectable in late F-type stars. [abridged]

==> fluid_numbers.tex <==
\begin{table}[h!]
    \centering
    \caption{Dimensionless numbers in the middle of the convective zone, $\tau_\mathrm{conv}$, and $r_c - r_0$ penetration depth. 
    %{\color{red} Also we should discuss the choice of probing the middle of the convective zone for the Rayleigh number : the Rayleigh bump is between 0.94 and 0.96 $R_\star$ and I take the mean value between 0.92 and 0.94 $R_\star$. This is important only for $Ra$ as for $Ra^*$ we consider the peak $dS/dr$ value in the convective zone.}
    }
    \begin{tabular}{ccccc}
    \hline \hline
    Case & F1a & F1b & F3 & F5 \\
    \hline
    $Re$ & 20 & 73 & 39 & 64 \\
    $Ro_f$ & 4.1 & 6.1 & 1.9 & 1.4 \\
    $Ro_s$ & 5.8 & 6.8 & 2.0 & 1.2  \\
    $Ro_c$ & 2.3 & 2.0 & 0.8 & 0.6 \\
    $Ra$ & \num{1.5e3} & \num{1.2e4} & \num{6.4e3} & \num{2.5e4} \\
    $Ta$ & \num{1.1e3} & \num{1.2e4} & \num{4.0e4} & \num{3.1e5} \\
    $Ra^*/Ra_c$ & 14.3 & 23.9 & 4.5 & 2.8 \\
    $\tau_\mathrm{conv}$ (day) & 4.8 & 4.1 & 4.8 & 4.8 \\
    $\overline{d}_\mathrm{ov}$ ($H_p$) & 0.22 & 0.23 & 0.18 & 0.15 \\
    \end{tabular}
    \label{tab:dimensionless_numbers}
\end{table}

==> model_summary.tex <==
\begin{table*}[]
    \centering
    \caption{Global properties for the considered cases.}
    \begin{tabular}{ccccc}
    \hline \hline
    Case & F1a & F1b & F3 & F5 \\
    \hline
    ($N_r$, $N_\theta$, $N_\phi$) & (1205, 512, 1024) & (1205, 1024, 2048) & (1205, 1024, 2048) & (1205, 1024, 2048) \\
    $\Omega_0$ ($\Omega_\odot$) & 1 & 1 & 3 & 5 \\
    $\nu_\mathrm{top}$ (cm$^2$/s) & \num{3.5e13} & \num{1.05e13} & \num{1.75e13} & \num{1.05e13} \\
    $\kappa_\mathrm{top}$ (cm$^2$/s) & \num{1.4e14} & \num{4.2e13} & \num{7e13} & \num{4.2e13} \\
    $r_t$ (cm) & \num{8.9e10} & \num{8.9e10} & \num{8.9e10} & \num{8.9e10} \\
    Longest time series (day) & 117 & 52 & 48 & 130 (280) \\
    \end{tabular}
    \tablefoot{
    The last row of the table specifies the longest $v_r$ time series we have for each case (with a time sampling $dt$ below 1250s to keep the Nyquist frequency of the series above $N_\mathrm{max} = 400$~$\mu$Hz, see Sect.~\ref{sec:igw_spectrum}.), with outputs saved for one depth every 1\% of the stellar radius. The value between parenthesis in the F5 case correspond to the length of the time series for which we save outputs only at $r = 0.13 \, R_\star$. This time series is used in Sect.~\ref{sec:period_spacing} and \ref{sec:splittings}.  
    }
    \label{tab:model_summary}
\end{table*}
